Full-Stack, Real-System Quantum Computer Studies: Architectural Comparisons and Design Insights

In recent years, Quantum Computing (QC) has progressed to the point where small working prototypes are available for use. Termed Noisy Intermediate-Scale Quantum (NISQ) computers, these prototypes are too small for large benchmarks or even for Quantum Error Correction, but they do have sufficient resources to run small benchmarks, particularly if compiled with optimizations to make use of scarce qubits and limited operation counts and coherence times. QC has not yet, however, settled on a particular preferred device implementation technology, and indeed different NISQ prototypes implement qubits with very different physical approaches and therefore widely-varying device and machine characteristics. Our work performs a full-stack, benchmark-driven hardware-software analysis of QC systems. We evaluate QC architectural possibilities, software-visible gates, and software optimizations to tackle fundamental design questions about gate set choices, communication topology, the factors affecting benchmark performance and compiler optimizations. In order to answer key cross-technology and cross-platform design questions, our work has built the first top-to-bottom toolflow to target different qubit device technologies, including superconducting and trapped ion qubits which are the current QC front-runners. We use our toolflow, TriQ, to conduct {\em real-system} measurements on 7 running QC prototypes from 3 different groups, IBM, Rigetti, and University of Maryland. From these real-system experiences at QC's hardware-software interface, we make observations about native and software-visible gates for different QC technologies, communication topologies, and the value of noise-aware compilation even on lower-noise platforms. This is the largest cross-platform real-system QC study performed thus far; its results have the potential to inform both QC device and compiler design going forward.

==> arch_implications.tex <==
1. Influence of qubit technology on program success rates:
Gate set: ion traps have arbitrary rotations, superconducting qubits have pi/2 pulses. More pulses needed for 1Q gates.
Ion cannot perform XXs in parallel. Hence, computation is longer and there may be more chances for noise corruption in larger systems.
Programs may have specific sequences of gates which could be pulse-optimized for each machine. Exposing pulse level details and control will be useful for NISQ systems.

It is also useful to have arbitrary rotations possible in H/W. Reduces program length.

Device error rates: The most crucial factor for current systems. Improving device error rates and error variance will be they key to enable larger computations. Important to focus on all three error rates 1Q, 2Q and RO. Having imbalance among them will hurt programs.

Deviec topology: Right appl. machine topology match is important. Systems with richer topology have higher program success rate. It is more useful to have a small number of qubits with dense conenctivity rather than a large number of  weak qubits which are sparsely connected. At least two real applications have been demonstrated on small systems (LPN, Johri).

Noise-adaptivity matters across systems. Noise phenomea is expected to stay.

4. Coherene time considerations are less important for current machines, because programs are limited by operational error rates.

done
-----
6. Propagating micro-architecture details upwards in the stack and making compilation choices based on them enables much higher program success rates.
7. QC is not ready for a device independent abstraction layer

5. It is useful for the ISA to expose more native operations and allow the compiler to optimize them. e.g., on any universal set of native gates, we can construct device dependent CNOT gates.
Compilers can use IR which is device independent CNOT + 1Q abstraction for high level  optimization, but all optimizations should be driven by microarch. considerations.


==> deleted.tex <==

\begin{figure*}[t]
\centering
\subfloat[Qubit, fundamental gates and ISAs of 3 vendors]
{
    \includegraphics[scale=0.45]{figs/qubits_table.png}
    \label{fig:qubit_prop}
}
\qquad
\subfloat[Noise properties and qubit Connectivity of 5 devices]
{
    \includegraphics[scale=0.4]{figs/noise_topology_table.png}
    \label{fig:device_prop}
}
\subfloat[Daily variations in CNOT error rates on IBMQ14]
{
    \includegraphics[scale=0.4]{figs/cx_daily_var.pdf}
    \label{fig:ibm_cx_var}
}
\caption{(a) describes the qubit technology used by 3 vendors. The vendor provides a universal gate set which can be used to implement higher-level operations such as the CNOT gate. (b) shows the devices used in our study, their one-qubit (1Q), two-qubit (2Q), readout (RO) error rates and topology of the qubit connections in the device. Each black circle represents a qubit and the edges denote the permitted hardware 2Q operations. The white qubits in Agave were unavailable during our experiments.
(c) shows the daily variations in CNOT error rates in IBMQ14. The gates have variable error rates across time and qubits in the system.}
\label{fig:machines}
\end{figure*}







\section{Overview of our Toolflow}
Figure \ref{fig:toolflow} shows the \compilername toolflow. To study application performance across devices and understand the impact of architecture and ISA design choices, we start with a high-level language input which is independent of the implementation. This allows us to apply the same optimization passes for different devices. 

To study
\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.5]{figs/framework_initial.png}
    \caption{Overview of the \compilername toolflow. 
    %Qubit mapping, gate scheduling and CNOT routing phases are dependent on the program instructions, machine topology and noise properties.
    }
    \label{fig:toolflow}
\end{figure*}

Our toolflow uses the Scaffold language, which extends C with quantum gates. Scaffold programs are independent of the machine and vendor ISA. The ScaffCC compiler \cite{scaffcc1, scaffcc2} is the frontend which generates input for our backend compiler. It decomposes high-level operations such as the Toffoli gate, inlines functions, unrolls loops and produces an LLVM Intermediate Representation (IR) \cite{llvm} of the program. Current NISQ hardware supports only small sized programs, hence we can fully flatten programs for optimization. The IR version of the program includes the qubits required for each operation and the data dependencies between operations. The IR expresses the computation using a universal set of common 1Q operations, namely $H$, $X$, $Y$, $Z$,$S$, $S^\dagger$, $T$, $T^\dagger$, $R_x(\theta)$, $R_y(\phi)$ and $R_z(\lambda)$, and 2-qubit CNOT gates.  
For example, Figure \ref{fig:bv_ir} shows an example IR for the Bernstein-Vazirani algorithm on 4 qubits (BV4) \cite{bernsteinvazirani}, a common benchmark algorithm featured in several QC platforms \cite{cirq, projectq1, bv_rigetti}.
QC programs are usually compiled for a fixed input size. ScaffCC resolves all classical control dependencies and the IR includes only quantum operations. 





%We generate executable code optimized for the microarchitecture in terms of the vendor provided ISA. Our toolflow is easily extensible. To configure our compiler for a new vendor/device, the vendor needs to supply a set universal ISA gates and the qubit topology. Since CNOTs and other 1Q gates can be generated from a universal gate set, we can compile Scaffold programs into communication and 1Q gate optimized code with this information.  To obtain benefits from noise-adaptive compilation, the vendor should provide reliablity data for each hardware gate on the system. Both superconducting and trapped ion qubits are calibrated daily to adjust the gate time to fluctutations in environment temperature and other sources of noise. These calibration runs routinely collect the reliability data required by our compiler.Across the three vendors we have seen that differences in benchmarking and calibration methods do not significantly influence our compiler's performance.


qubit mapping
------------

\subsection{Qubit Mapping}
To perform qubit mapping, our compiler sets up an SMT optimization problem with variables that specify the qubit mapping and constraints that associate mappings with reliablites using the matrices $R_{2Q}$ and $R_{RO}$ computed earlier. The solver finds a mapping which maximizes the reliability for all 2Q and RO operations.

Let $Q$ be the set of program qubits and $H$ be the set of hardware qubits. 
For $q \in Q$, $q.h$ is the hardware qubit assigned to the program qubit $q$. 
Let $G$ be the set of operations in the program. This set is composed of $G_1$, the set of single-qubit gates, $G_2$, the set of 2-qubit gates and $G_{RO}$, the set of readout operations. For each gate $g$ in the program, the reliability is denoted by ($g.\epsilon$).
\subsubsection{Constraints}
{\noindent \bf Qubit Mapping Constraints:} Constraint \ref{c1}, guarantees that all program qubits are mapped to actual hardware qubits. Constraint \ref{c2} guarantees that each program qubit is assigned a distinct hardware location.
\begin{align}
    \forall q \in Q : 0 \le q.h < |H| \label{c1}\\
    \forall q_i, q_j \in Q : q_i.h \neq q_j.h \label{c2}
\end{align}

{\noindent \bf Reliability Constraints:} 
These constraints associate qubit mappings with the reliability information of 2Q and RO operations. Let $g.\epsilon$ denote the reliability score for the operation $g$. 

For each two qubit gate $g \in G_2$, with control qubit $c$ and target qubit $t$, if the control and target qubits are assigned to hardware qubits $h_i, h_j \in H$, the reliability assignment is:
\begin{align}
    c.h = h_i \land t.h = h_j \Rightarrow g.\epsilon = R^{2Q}_{h_i, h_j}. 
\end{align}

For trapped ion systems with full connectivity qubit swapping is not required and $R^{\text{2Q}}$ specifies the  reliabilities of the 2Q (Ising) operations for every pair of ions.

For each readout operation in $G_R$, we associate reliabilities as 
\begin{align}
    \forall g \in G_{RO}: \forall h_i \in H: g.h = h_i \Rightarrow g.\epsilon = R^{RO}_{h_i}.
\end{align}

\subsubsection{Objective Function}
The ideal reliability objective is the product of all reliabilities of all 2Q and RO operations in the program. Under this objective, the optimization is to find the mapping which maximizes: 
\begin{align}
 \prod_{\forall g \in G_{RO} \cup G_{2Q}} g.\epsilon.
\end{align}
Since the SMT solver requires linear operations, following \cite{asplos}, this objective can be converted into an additive linear objective function by considering the logarithm of the gate reliabilities. This changes the objective function to
\begin{align}
 \sum_{\forall g \in G_{RO} \cup G_{2Q}} \log (g.\epsilon)
\end{align}

Optimizing reliability places qubits at hardware locations with high CNOT and readout reliability. It indirectly optimizes qubit movement because CNOT gates between program qubits placed at non-adjacent hardware qubits have low reliability. \cite{asplos} shows that SMT optimization with this objective scales to programs with 32 qubits. 

To scale SMT methods further, we use an objective function where the reliability is computed as 
\begin{align}
     \min_{\forall g \in G_{RO} \cup G_{2Q}} (g.\epsilon).
\end{align}
This objective says that the reliability of an qubit mapping is the reliability of its worst gate. Under this objective the optimization is to find a qubit mapping where the reliability of the worst gate is as high as possible. We use this reliability function for programs with higher qubit count because the error variance in larger systems will reduce and it will be sufficient to find mappings where the worst qubits and gate are avoided. 
Using the min-based objective instead of a summation allows a faster SMT implementation. The min-based objective can be implemented by constraining that all gates have a reliability greater than a threshold $t$ and checking if the optimization is satisfiable. The best value of $t$ can be computed by binary search in $[0,1]$. This implementation allows the SMT solver to prune candidate solutions fast: if it maps two qubits and finds that a gate has lesser reliability than $t$, it can discard the mapping. In contrast, for the summation based method, the solver has to place all qubits and evaluate the summation over all the 2Q and RO operations. This reliablity function provides up to three orders of performance improvement over \cite{asplos} and is especially useful for problems where \cite{asplos} fails to compute a solution.

To compute a qubit mapping with the SMT solver, we set up an optimization problem using this objective along with the qubit mapping and reliability constraints. The reliability constraints associate the $g.\epsilon$ variables with the qubit mapping variables and the solver finds a mapping which maximizes reliability.

----------

%effect of average gate error rate.
\paragraph{Importance of average operation reliability}
Consider the HS4 benchmark where two pairs of program qubits perform 2Q gates with each other (see Figure \ref{fig:benchmarks}). Our compiler maps this benchmark without any swap operations for all the machines. On HS4, IBM machines have $5$x higher success rate than Rigetti because they have lesser average 1Q, 2Q and RO error rates. 
HS2 and QFT can also be mapped to all devices without swaps. Here we see that Rigetti has marginally better performance than IBM. HS2 and QFT exercise only hardware 2Q unit. Rigetti's best hardware CZ gate is comparable in performance to IBM. However, Rigetti's 2Q gate is bi-directional while IBM is uni-directional. Hence additional single qubit gates are required on IBM, degrading its performance marginally.
For the Toffoli, Fredkin, Or and Peres benchmarks, IBMQ5 and UMD TI both allow the benchmark to be mapped without any swaps. In these cases, ion traps offers the best performnce because its gate errors are substantilly lower.

\paragraph{Importance of reducing noise variability}
Consider the executions of IBMQ14 and IBMQ16. For all benchmarks, these two devices expose the same device topology and gate set, but IBMQ14 has higher variance in gate error rates compared to IBMQ16. This is partly because IBMQ14 is a new machine and the qubits and gate are still being tuned and stabilizied. Across all benchmarks, we can see that IBMQ14 has lower success rate than IBMQ16. For HS2 and HS4, Rigetti's performance degrades drastically for HS4 compared to HS2 while for the IBM devices HS4 underperforms HS2 only mildly, owing to lesser noise variability. 

\paragraph{Impact of device connectivity on benchmark performance}
Consider the executions of Toffoli, Fredkin and Or benchmarks on IBMQ5 and IBMQ16. These benchmarks can be mapped without swaps on IBMQ5, while they require at least one swap on IBMQ16. Correspondingly IBMQ16 offers lower success rates for these benchmarks. On Rigetti these benchmarks fail because the high error rates degrade programs with even a small number of swaps.

Similarly, the BV4 benchmark can be mapped to the IBMQ16 device without any swaps. It requires one swap on IBMQ5 and one swap on Rigetti. Consequently, IBMQ16 outperforms the other two systems on this benchmark. 

UMD TI has full connectivity and is therefore oblivious to program communication behavior. It obtains consistently high success rates on all benchmarks.

To the best of our knowledge, our work is the first to perform cross-vendor benchmarking of this scale, using a high level language compiler. This experiment shows that it is important to improve systems across multiple fronts, by minimize gate error rates, reducing the noise varibility across gates, and improving the device connectivity to support complex program communication patterns. 

==> methodologyOLD.tex <==
\section{Overview of our Toolflow}
Figure \ref{fig:toolflow} shows the \compilername tooflow. To target diverse QC systems, we designed our toolflow to accept high-level language programs as input. Our toolflow uses the Scaffold language which can represent QC programs using high-level operations which are specified in a device and vendor-independent manner. Using the ScaffCC compiler\cite{scaffcc1, scaffcc2}, our toolflow converts Scaffold code into an LLVM intermediate representation (IR) which consists of single and two-qubit gates. Figure \ref{fig:bv_ir} shows the IR for the Bernstein-Vazirani algorithm. ScaffCC automatically decomposes high-level operations such as Toffoli gates into their representations using 1 and 2-qubit gates. The IR version of the program includes the qubits required for each operation and the data dependencies between operations. Since QC programs are usually compiled for a fixed input size, ScaffCC also resolves all classical control dependencies and produces IR which includes only quantum operations. 

We build a compiler which transforms this IR into executable code through a set of configurable passes. Inspite of the diversity in the systems, we observe that the key phases of compilation can represent the IR using a common gate set while still applying transformations based on low-level device properties. These passes accept machine properties such as noise rates and topology as input, allowing us to study various machine types in a uniform manner. After these transformations, device specific passes can be applied to produce optimized code for the target machine. These passes can be configured using a gate set, allowing us to study good choices for software-visible gates in a vendor's stack.
Although we unify various parts of the compilation across devices, in our experiments we show that our toolflow is superior to vendor compilers, and extracts the best performance from the hardware.

We use a flexible representation of a QC machine. The representation includes 3 components: ISA, topology and noise information. To study the impact of vendor ISAs, our compiler can generate code for different target gate sets and includes options to optimize gate sequences, allowing us to evaluate the merits and demerits of each ISA. To understand the impact of gate topology and noise, we build a uniform representation of the machine, which includes specifices the operations reliablities including topology and noise considerations. Using this representations, use a set of common qubit mapping, gate scheduling and routing passes which optimizes the executable for topology and noise properties of the device, allowing us to obtain the best benchmark performance for applications.

\begin{figure*}[h]
    \centering
    \includegraphics[scale=0.5]{figs/framework_initial.png}
    \caption{Overview of the \compilername toolflow. 
    %Qubit mapping, gate scheduling and CNOT routing phases are dependent on the program instructions, machine topology and noise properties.
    }
    \label{fig:toolflow}
\end{figure*}
Figure \ref{fig:toolflow} shows the \compilername toolflow. 
Our toolflow uses the Scaffold language, which extends C with quantum gates. Scaffold programs are independent of the machine and vendor ISA. The ScaffCC compiler \cite{scaffcc1, scaffcc2} is the frontend which generates input for our backend compiler. It decomposes high-level operations such as the Toffoli gate, inlines functions, unrolls loops and produces an LLVM Intermediate Representation (IR) \cite{llvm} of the program. Current NISQ hardware supports only small sized programs, hence we can fully flatten programs for optimization. The IR version of the program includes the qubits required for each operation and the data dependencies between operations. The IR expresses the computation using a universal set of common 1Q operations, namely $H$, $X$, $Y$, $Z$,$S$, $S^\dagger$, $T$, $T^\dagger$, $R_x(\theta)$, $R_y(\phi)$ and $R_z(\lambda)$, and 2-qubit CNOT gates.  
For example, Figure \ref{fig:bv_ir} shows an example IR for the Bernstein-Vazirani algorithm on 4 qubits (BV4) \cite{bernsteinvazirani}, a common benchmark algorithm featured in several QC platforms \cite{cirq, projectq1, bv_rigetti}.
QC programs are usually compiled for a fixed input size. ScaffCC resolves all classical control dependencies and the IR includes only quantum operations. 

\begin{figure*}[t]
\subfloat[IR for Bernstein-Vazirani with 4 qubits (BV4)]
{
    \includegraphics[scale=0.4]{figs/BV_IR.png}
    \label{fig:bv_ir}
}
\subfloat[Two mappings for BV4 on IBMQX4]
{
    \includegraphics[scale=0.6]{figs/MappingExample.png}
    \label{fig:bv_mapping}
}

    \caption{The intermediate representation of input program uses program qubits and has 1Q, 2Q and RO operations.  }
    \label{fig:bv_example}
\end{figure*}

\subsection{Compilation Tasks and Objective} 

The backend compiler performs four tasks to optimize the IR for the target architecture. First, it \textbf{maps the qubits} in the program onto distinct hardware qubits. Figure \ref{fig:bv_mapping} shows an example  placement for the program qubits $p_0$-$p_3$ in the BV4 IR onto the qubits in the IBMQX4 machine. Second, it \textbf{schedules the gates} to respect data dependencies in the program. For BV, this step corresponds to executing the first set of X and H gates, followed by the CNOTs, the final H gates and the readout operations. For the naive mapping, the first CNOT is performed between $p_0$ and $p_3$ which is not supported between the corresponding hardware qubits. For such architectures with limited connectivity, the compiler \textbf{inserts routing operations} to move the CNOT qubits into adjacent locations. On superconducting architectures, these operations are SWAP gates which move qubits one hop at a time. After swapping $p_2$ and $p_3$, all the program CNOTs can be performed. Notice that the compiler can determine the optimized mapping in Figure \ref{fig:bv_mapping}  and avoid this swap operation. Finally, the compiler uses  the \textbf{emits optimized executable code} in the vendor ISA. 

On real QC devices, because of the experimental noise, code is executed thousands of times in succession and the outputs are summarized in the form of a probability distribution over bitstrings. We refer to the experimentally measured probability of the correct bitstring as {\em success rate}. The primary design goal of our compiler is to maximize the success rate, i.e., we maximize the likelihood of a program's success on a target device.

To maximize success rate, our toolflow computes a {\em reliability} score for an executable. The reliability is an an estimate of the success rate of the program on the target architecture. A simple measure of reliability for a program with $n$ operations is $(1-e)^n$, where $e$ is the average gate error rate in the system. Using this estimate, we can reduce $n$ by mapping communicating qubits close together and by applying gate-level optimizations. However, Figure \ref{fig:device_prop} and \ref{fig:ibm_cx_var}, device error rates are different for each operation type, and exhibit variability even within an operation type across qubits and time. Given a hardware mapped IR, such as the naive or optimized mappings in Figure \ref{fig:bv_mapping}, \compilername calculates the reliability as the product of the reliability of each gate and readout operation. Qubit mappings and swap sequences which use error-prone gates have a lower reliablity score compared to mappings which optimize communication and adapt placement to use the most reliable hardware. Using reliability considerations to determine the qubit mapping and CNOT routing paths, and perform low-level 1Q optimizations, \compilername optimizes the program to execute with high success rate.

\subsection{Compilation Passes}
{\noindent \bf Noise-Adaptive Qubit Mapping: } Using noise data from the vendor, \compilername performs a pairwise qubit reliablity computation to determine the the reliablity of a CNOT gate between every pair of qubits, including the SWAP gates necessary along the path. We formulate an SMT optimization problem which considers program instructions, the computed reliablity matrix and readout errors for every hardware qubit to determine an optimal qubit mapping which maximizes reliability.

{\noindent \bf Gate Scheduling and CNOT Routing: } Next, \compilername schedules gates in topologically sorted order to respect data dependencies. Using the initial qubit mapping, gate schedule and machine connectivity, \compilername identifies the CNOTs which require routing operations. For each such CNOT, \compilername uses a greedy algorithm to choose the best routing path and inserts SWAP gates in the IR.

{\noindent \bf Code Generation and Low-level Optimization: } First, using the qubit mapping, each IR operation is re-written to use hardware qubits instead of program qubits. The IR gates are then decomposed into the gate set supported by the device. SWAP gates are decomposed to CNOTs or ISA 2Q and 1Q operations depending on the ISA. Then CNOTs (including any CNOTs generated from SWAPs) are decomposed into the ISA supported gates. On devices where 2Q operations can be performed only in one direction (IBM), the directions for 2Q gates are are corrected in software by inserting additional 1Q operations. At this stage all operations in the IR are hardware mapped and respect the constraints of the device topology and directions. To further optimize code, \compilername extracts all sequences of 1Q gates. On IBM and ion trap, Z rotations are inexpensive compared to X and Y rotations. \compilername leverages this difference to maximize the number of Z rotations using quaternions.
Finally, \compilername translates the IR operations to a vendor provided format for execution on the target device.

\section{SMT Optimization for Qubit \\ Mapping}
\subsection{Notations and Design Choices}
Let $Q$ be the set of program qubits and $H$ be the set of hardware qubits. The topology of the hardware qubits is specified by a graph where $T(H, E)$, where each edge $e = (h_i, h_j) \in E$, indicates a hardware 2Q gate between $h_i$ and $h_j$. $T$ can be directed or undirected depending on the device. 

For $q \in Q$, $q.h$ is the hardware qubit assigned to the program qubit $q$. 
Let $G$ be the set of operations in the program. This set is composed of $G_1$, the set of single-qubit gates, $G_2$, the set of 2-qubit gates and $G_{RO}$, the set of readout operations. For each gate $g$ in the program, the reliability is denoted by ($g.\epsilon$).

Figure \ref{fig:machines} shows that 1Q gate errors are much lower than 2Q and RO operations, hence we do not optimize qubit mappings according to them. Moreover, sequences of 1Q gates can be optimized in a later compiler pass (Section \ref{}). 
Prior work \cite{asplos} showed that optimizing operations error rates is more important than coherence times on IBMQ16. On trapped ion systems, the coherence time is so high that the program success rates are only limited by gate errors. Their current coherence time of 1.5s can support 1000s of 2Q operations, but the gate errors of 1-3\% and readout errors prevent long gate sequences. Based on these observations, we choose to drive the qubit mapping decisions according to operation reliablities alone.

\subsection{Constraints}
{\noindent \bf Qubit Mapping Constraints:} Constraint \ref{c1}, guarantees that all program qubits are mapped to actual hardware qubits. Constraint \ref{c2} guarantees that each program qubit is assigned a distinct hardware location.
\begin{align}
    \forall q \in Q : 0 \le q.h < |H| \label{c1}\\
    \forall q_i, q_j \in Q : q_i.h \neq q_j.h \label{c2}
\end{align}

{\noindent \bf Reliability Constraints:} 
These constraints associate qubit mappings with the reliability information of 2Q and RO operations. Let $g.\epsilon$ denote the reliability score for the operation $g$. For each readout operation in $G_R$, we associate reliabilities as 
\begin{align}
    \forall g \in G_{RO}: \forall h_i \in H: g.h = h_i \Rightarrow g.\epsilon = R^{RO}_{h_i}.
\end{align}
$R^{RO}$ is a vector with the reliability of the RO operations for each hardware qubit in the device. In QC literature, this value is called the single-shot readout fidelity of a hardware qubit.

For 2Q operations, we perform an all-pairs reliablity computation using the 2Q gate fidelities reported by the vendor. For each pair of hardware qubits $h_i$ and $h_k$, we determine a ``most reliable'' routing path from $h_i$ to $h_k$ using Dijkstra's algorithm. 
We construct a graph where each node is a hardware qubit with edges denoting the permitted 2Q operations. Each edge $(u,v)$ with 2Q gate fidelity $f$ is assigned an edge weight $-\log f^3$ since one swap on IBM and Rigetti machines requires 3 2Q gates \footnote{For IBM machines, we also include the fidelity of any extra 1Q operations required for gate direction corrections.}. Computing shortest paths on this graph provides the most reliable swap sequence from $h_i$ to $h_k$. To find the reliability of a CNOT from $h_i$ to another node $h_j$, we find the reliabilities to each neighbor $h_k$ of $h_j$. We select the $h_k$ which has the highest product of $h_i$ to $h_k$ reliablity and CNOT $h_k$, $h_j$ reliablity and denote the product reliablity as $R_{h_i, h_j}^{2Q}$. 

For each two qubit gate $g \in G_2$, with control qubit $c$ and target qubit $t$, if the control and target qubits are assigned to hardware qubits $h_i, h_j \in H$, the reliability assignment is:
\begin{align}
    c.h = h_i \land t.h = h_j \Rightarrow g.\epsilon = R^{2Q}_{h_i, h_j}. 
\end{align}

For trapped ion systems with full connectivity qubit swapping is not required and $R^{\text{RO}}$ specifies the  fidelities of the 2Q (Ising) operations for every pair of ions.

\subsection{Objective Function}
The ideal reliability objective is the product of all reliabilities of all 2Q and RO operations in the program. Under this objective, the optimization is to find the mapping which maximizes: 
\begin{align}
 \prod_{\forall g \in G_{RO} \cup G_{2Q}} g.\epsilon.
\end{align}
Since the SMT solver requires linear operations, following \cite{asplos}, this objective can be converted into an additive linear objective function by considering the logarithm of the gate reliabilities. This changes the objective function to
\begin{align}
 \sum_{\forall g \in G_{RO} \cup G_{2Q}} \log (g.\epsilon)
\end{align}

Optimizing reliability places qubits at hardware locations with high CNOT and readout reliability. It indirectly optimizes qubit movement because CNOT gates between program qubits placed at non-adjacent hardware qubits have low reliability. \cite{asplos} shows that SMT optimization with this objective scales to programs with 32 qubits. 

To scale SMT methods further, we use an objective function where the reliability is computed as 
\begin{align}
     \min_{\forall g \in G_{RO} \cup G_{2Q}} (g.\epsilon).
\end{align}
This objective says that the reliability of an qubit mapping is the reliability of its worst gate. Under this objective the optimization is to find a qubit mapping where the reliability of the worst gate is as high as possible. We use this reliability function for programs with higher qubit count because the error variance in larger systems will reduce and it will be sufficient to find mappings where the worst qubits and gate are avoided. 

Using the min-based objective instead of a summation allows a faster SMT implementation. The min-based objective can be implemented by constraining that all gates have a reliability greater than a threshold $t$ and checking if the optimization is satisfiable. The best value of $t$ can be computed by binary search in $[0,1]$. This implementation allows the SMT solver to prune candidate solutions fast: if it maps two qubits and finds that a gate has lesser reliability than $t$, it can discard the mapping. In contrast, for the summation based method, the solver has to place all qubits and evaluate the summation over all the 2Q and RO operations. This reliablity function provides up to three orders of performance improvement over \cite{asplos} and is useful for problems where \cite{asplos} fails to compute a solution.

To compute a qubit mapping with the SMT solver, we set up an optimization problem using this objective along with the qubit mapping and reliability constraints. The reliability constraints associate the $g.\epsilon$ variables with the qubit mapping variables and the solver finds a mapping which maximizes reliability.

\section{Gate Scheduling and Noise-Adaptive Routing}
We schedule gates in a topologically sorted order from the IR's gate dependencies. This ensures that before a gate is executed, all its dependent gates are completed. Using the qubit mapping gate schedule, and hardware qubit topology, the compiler determines routing paths for CNOTs which do no operate on adjacent hardware qubits. This step is only required for architectures with sparse topology, such as those from IBM and Rigetti.

To route a CNOT, the compiler uses the most reliable path for the CNOT control and target qubit pair computed in the previous section.
For each CNOT in the scheduled order, the compiler uses best path and inserts the SWAP gates necessary to change the qubit mapping. For the subsequent CNOT, the compiler considers the updated qubit mapping.

\section{Code Generation and Low-level Optimization}
We divide code generation into 2 steps: gate decomposition and single qubit gate optimization. Gate decomposition breaks down the IR gates into the gates supported by the device. We perform this in three steps: swap decomposition, CNOT decomposition and gate direction implementation. First, any SWAP operations in the IR are broken down into 2Q gates. For IBM and Rigetti devices which  this is accomplished by the transformation shown in Figure \ref{}. Ion traps do not require swaps because of full connectivity. Next, all CNOTs in the IR are replaced by their ISA 2Q and 1Q equivalent code sequence shown in Figure \ref{fig:qubit_prop}. Finally, since IBM devices have directed CNOTs, our compiler checks whether the CNOTs in the IR are oriented in the correct direction. When the program requires a CNOT in the opposite direction, the compiler uses a standard transformation to reverse the gate ordering. 

At this stage, the IR is a mixture of ISA supported 2Q operations, and arbitrary 1Q gates. To decompose and optimize 1Q gates into the ISA suported 1Q gates, for each qubit, we extract continuous sequences of 1Q operations in the IR. Since 1Q operations are rotations, each 1Q gate in the IR can be expressed using a rotation quaternion which is a canonical representation using a 4D complex number. After translating the gates into quaternions, the quaternions are multiplied together to create a single arbitrary rotation. This arbitrary rotation is then expressed in terms of the ISA 1Q gates. On IBM, Rigetti and UMD TI gate sets, Z gates are allowed arbitrary angles. Further more, on IBM and UMD TI, Z gates are error-free: they are special gates which are implemented in classical hardware instead of manipulating the qubits. Hence, we use known techniques to express the quaternion as a product of 2 Z rotations and a single rotation along either X or Y axis.


==> results_old.tex <==


\section{Cross-Platform Benchmark Comparison}
We used \compilername to compile the 12 benchmarks for 5 systems. Our compiler optimizes the benchmarks on each system by using a combination of intelligent qubit mapping, routing 2Q operations, and optimizing the single qubit gates. Figure shows the success rate measured for each of the compiled executables. Some benchmarks are too large to be mapped onto the IBMQ5, Rigetti and Ion trap machines. These runs are marked ``S''. When a benchmark fails to execute on a platform because of large errors, the run is marked ``F''. In this experiment, the ion trap benchmarks were compiled without calibration data.
\textbf{Three factors collectively determine benchmark performance on an architecture: average operation reliability, noise variability, device connectivity}

%effect of average gate error rate.
\paragraph{Importance of average operation reliability}
Consider the HS4 benchmark where two pairs of program qubits perform 2Q gates with each other (see Figure \ref{}). Our compiler maps this benchmark without any swap operations for all the machines. IBM machines have $5$x higher success rate than Rigetti because they have lesser average 1Q, 2Q and RO error rates. 
For the Toffoli, Fredkin, Or and Peres benchmarks, IBMQ5 and ion trap both allow the benchmark to be mapped without any swaps. In all these cases, ion traps offers the best performnce because its gate errors are substantilly lower.

HS2 and QFT can also be mapped to all devices without swaps. Here we see that Rigetti has marginally better performance than IBM. HS2 and QFT exercise only hardware 2Q unit. Rigetti's best hardware CZ gate is comparable in performance to IBM. However, Rigetti's 2Q gate is bi-directional while IBM is uni-directional. Hence additional single qubit gates are required on IBM, degrading its performance marginally.

\paragraph{Importance of noise variability}
Consider the executions of IBMQ14 and IBMQ16. For all benchmarks, these two devices expose the same device topology and gate set, but IBMQ14 has higher variance in gate error rates compared to IBMQ16. This is partly because IBMQ14 is a new machine and the qubits and gate are still being tuned and stabilizied. Across all benchmarks, we can see that IBMQ14 has lower success rate than IBMQ16. For HS2 and HS4, Rigetti's performance degrades drastically for HS4 compared to HS2 while for the IBM devices HS4 underperforms HS2 only mildly, owing to lesser noise variability. 

\paragraph{Importance of device connectivity}
IBM and Rigetti's machines have low connectivity i.e., 2Q operations between distant pairs of qubits requires swaps. Each swap operations requires 3 native 2Q operations, resulting in high gate errors and poor performance for any benchmark which requires swaps. Ion trap has full connectivity and is therefore oblivious to program communication behavior. It obtains consistently high success rates on all benchmarks.

The BV4 benchmark can be mapped to the IBMQ16 device without any swaps. It requires one swap on IBMQ5 and one swap on Rigetti. Consequently, IBMQ16 outperforms the other two systems on this benchmark. Similarly, Toffoli, Fredkin, Or and Peres require no swaps and have high success rate on IBMQ5, while they require at least one swap on IBMQ16 and Rigetti. On Rigetti these benchmarks fail because the programs require a large number of swaps which cannot be executed with the device's high gate errors.
Similarly, adder has lower performance on IBMQ5, compared to IBMQ16, where it requires no swaps. 

To the best of our knowledge, our work is the first to perform cross-vendor benchmarking of this scale, using a high level language compiler. This experiment shows that it is important to minimize gate error rates, reduce noise varibility across gates, and improve device connectivity to support complex program communication patterns.

\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.35]{figs/expt/bench_all.png}
    \caption{Evaluation of 12 benchmarks on 5 systems. Benchmark performance varies drastically across systems and is heavily influenced by gate error rates, qubit connectivity, and application-machine toplogy match.}
    \label{fig:bench_perf}
\end{figure*}

\section{Leveraging Microarchitecture Information for Program Success}
\subsection{Evaluation on IBM Systems}
In this section, we compare the success rate of benchmark runs from our compiler vs. the IBM Qiskit compiler on 3 IBM machines. 

\subsubsection{Improvements in Success Rate over IBM Qiskit}
Figure \ref{fig:ibm_study} shows the success rate of the two methods on the 12 benchmarks. On these machines the margin of error in results from one run to the next is about 1-5\%. 

{\noindent \textbf{IBMQ5: }} On 3 benchmarks BV4, HS4 and Adder, our compiler outperforms Qiskit with up to 1.6X improvement in success rate. On the other benchmarks Qiskit and our compiler perform equally well, within the margin of error. 

{\noindent \textbf{IBMQ14: }}On IBMQ14, the gains for our compiler are more pronounced, with geomean 2.6x improvement, up to 12.9X. On BV4, BV6, BV8, HS4 and Adder, the dominant bitstring produced by Qiskit was wrong e.g, on BV4, the bitstring with highest occurences for Qiskit is ``1011'' with occurence rate $28\%$, while the correct bitstring ``1111'' occurs in only $4\%$ of the trials. In QC algorithm, the correct answer reported by an execution is usually the bitstring with the highest occurence rate.
On these 5 benchmarks, Qiskit's output cannot be used to determine the correct answers. In runs using our compiler, the correct answer occurs with high success rate and dominates all other answers. 

{\noindent \textbf{IBMQ16:}} On IBMQ16, we see similar improvements over Qiskit, with geomean improvement 3.0x and gains up to 28X on BV8 where Qiskit produces the correct answer in only $2\%$ of the trials.
\begin{figure*}[t]
    \centering

\subfloat[Experiments on IBMQ5]
{
    \includegraphics[scale=0.6]{figs/expt/succ_qx4_new.png}
    \label{fig:ibmq_5_compare}
}
\subfloat[Experiments on IBMQ14]
{
    \includegraphics[scale=0.6]{figs/expt/qmel_qiskit_compare.png}
    \label{fig:ibmq_14_compare}
}
\subfloat[Experiments on IBMQ16]
{
    \includegraphics[scale=0.6]{figs/expt/ibmqx5_qiskit_compare.png}
    \label{fig:ibmq_16_compare}
}
    \caption{Experirments on 3 IBM Devicecs. In IBMQ14 and IBMQ14, we obtain Xx improvement in success rate over the IBM Qiskit compiler.}
    \label{fig:ibm_study}
\end{figure*}

\subsubsection{Reasons for Success Rate Improvement}
Across all executions, we noticed that Qiskit always allocates the first few qubits on the device, without considering their error rates. We also confirmed this in its open source code base. Whenever the CNOT or readout rates of these qubits are high (error rates fluctuate by as much as $9$x), it further degrades Qiskit's performance. Our compiler modifies the qubit mapping to use the best CNOT and readout operations available in hardware.
\textbf{add picture showing mappings}

Figure \ref{fig:ibm_cx_study} shows the number of CNOTs used by Qiskit and our compiler on the 12 benchmarks, on the IBMQ16 machine. We see that our compiler uses up to geomean Xx lesser CNOT operations than Qiskit. Qiskits uses a large number of CNOTs because it chooses qubit mappings without optimizing for qubit communication.  Each extra SWAP operation for communication results in 3 CNOTs. Since CNOTs have high error rates, our compiler obtains large gains in success rate by reducing their usage. 

Our compiler also optimizes single qubit gate sequences and maximizes the use of Z rotations which are inexpensive for IBM's qubits. This improves the sucecess rate over an unoptimized version by up to $10\%$. Our workload has relatively few single qubit operations. On workloads from quantum chemistry such as Ising model (too large to execute on current systems) where more than $80\%$ of the operations are single qubit gates, we expect this optimization to be more useful.

Overall, on IBM devices, we see that optimizing for microarchitecture features such as noise and device topology provides significant benefits in success rate. 
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.6]{figs/expt/cx_qx5.png}
    \caption{CNOT counts for Qiskit and \compilername on IBMQ16. Our compiler obtains XX improvements in CX count, which translates to improvements in success rate.}
    \label{fig:ibm_cx_study}
\end{figure}
\subsection{Evaluation on Rigetti Agave}
Figure \ref{fig:rigetti_study} shows the success rates obtained using our compiler and Rigetti's Quil compiler on 4 benchmarks on Rigetti 4-qubit device. All other benchmarks either failed to execute correctly or were too large to be mapped onto the device. Our compiler obtains up to 1.9x improvement over the Quil compiler (geomean 1.46x). The mapping and swap operations used by both compilers for BV4 is shown in Figure \ref{}. BV4 requires one swap on this architecture because the program qubit $p_3$ is the target of CNOTs from three qubits, but the architecture only supports qubits with connectivity to 2 other qubits. Quil doesn't use noise data, hence it performs the swap using an less reliable hardware CZ gate. Our compiler performs the swap on the best hardware CZ gate and therby obtains improvements in success rate. 
Similarly, on HS2 and QFT our compiler chooses the best hardware CZ and readout units to perform the operations.

\textbf{1q gate count point?} 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figs/expt/succ_rigetti.png}
    \caption{Experiments on Rigetti Agave}
    \label{fig:rigetti_study}
\end{figure}

\textbf{add visuals of mapping}

\subsection{Evaluation on UMD Ion Trap}
Our compiler is the first high level language compiler for the trapped ion system. To map programs to this machine, the system developers use a default mapping where the program qubit with id $i$ is mapped to hardware qubit (ion) $i$. 
Figure \ref{fig:tion_baseline} shows the performance of the benchmarks using this mapping in our compiler, with and without 1Q gate optimization. To the best of our knowledge, this is the first experiment to report success rates of high-level language programs on this machine.  We can see that the success rates of all benchmarks are high on this machine, and 1Q gate optimization improves success rate by geomean 2.6\% over the default mapping, with up to 8.9\% improvement on the Fredkin benchmark. The improvement is much higher than the variability due to noise on this machine ($<1\%$ variability across runs of the same benchmark). Our compiler obtains these  improvements because it leverages the properties of native 1Q gates on this device. It maximizes the use of classically implemented Z rotations wherever possible, instead of using X and Y rotations which require laser control pulses, and hence improves success rate.

Figure \ref{fig:tion_noise_aware} compares the optimized default mapping and a noise-adaptive mapping using a mix of benchmarks. 



\begin{figure*}
    \centering

\subfloat[Single-qubit gate optimization]
{
    \includegraphics[scale=0.5]{figs/expt/tion_baseline.png}
    \label{fig:tion_baseline}
}
\subfloat[Noise-adaptive Compilation]
{
    \includegraphics[scale=0.5]{figs/expt/tion_noise_aware.png}
    \label{fig:tion_noise_aware}
}
    \caption{Expts on ion trap}
    \label{fig:tion_study}
\end{figure*}

\textbf{add plot of succ rate large if we get it}
\textbf{add visual of comparison}

\section{Scalability Studies}




